Detecting Abrupt Changes in Sequential Pairwise Comparison Data

The Bradley-Terry-Luce (BTL) model is a classic and very popular statistical approach for eliciting a global ranking among a collection of items using pairwise comparison data. In applications in which the comparison outcomes are observed as a time series, it is often the case that data are non-stationary, in the sense that the true underlying ranking changes over time. In this paper we are concerned with localizing the change points in a high-dimensional BTL model with piece-wise constant parameters. We propose novel and practicable algorithms based on dynamic programming that can consistently estimate the unknown locations of the change points. We provide consistency rates for our methodology that depend explicitly on the model parameters, the temporal spacing between two consecutive change points and the magnitude of the change. We corroborate our findings with extensive numerical experiments and a real-life example.

==> 07_exp_v0.tex <==
\section{Experiments: Backup}
\label{sec0:experiment}

% Compare the numerical performance of:

% \begin{enumerate}
%     \item DP with local refinement.
%     \item WBS with loglikelihood.
%     % \item Fused lasso. 
%     \item CUSUM-like method in, e.g., \cite{Hohle2010}.
% \end{enumerate}
In this section, we will demonstrate the advantage of our proposed method, i.e., DP with local refinement, from two perspectives. First, we show that a likelihood-based method would be more accurate than non-likelihood-based methods by considering the simplest setting where there is only one change point in the data. Second, in the scenario of multiple change points, we show that DP with local refinement is better than WBS in the sense that it gives more accurate localization with less tuning parameters.



\subsection{Single change point: likelihood is better than Borda count}
\label{sec0:experiment_single_cp}
\paragraph{Methods.} When it is known that there is only one change point $\eta$, the optimization problem \eqref{eq:P_hat_bt} has a simpler form
\begin{equation}
    \hat{\eta} = \argmin_{t\in (0,T)} \mathcal{R}_{BT}(t;(0,T]),
\end{equation}
where $\mathcal{R}_{BT}(t;(0,T]) = L(\hat{\bbrtheta}((0,t)),(0,t)) + L(\hat{\bbrtheta}([t,T]),[t,T])$ and $L(\bbrtheta,\mclI)$ is given in \Cref{eq:likelihood}. We can show the consistency of $\hat{\eta}$ by simpler arguments than \Cref{thm:consistency_bt}, see \Cref{prop:bt_single_cp} in the appendix. In fact, $\mathcal{R}(t;(0,T])$ is the the generalized likelihood ratio (GLR) statistic and idea of GLR screening works well for many models. For instance, it is a classical result in change point literature that when the data $\{Y_t\}_{t\in [T]}$ comes from a univariate mean model $Y_t=\mu_t + \epsilon_t$ where $\epsilon_t$ is Gaussian noise, the GLR screening gives optimal localization \citep{wang2018univariate}. 

For multi-variate Gaussian observations with known variance, it can be shown (see \Cref{prop:multi-Gaussian}) that the GLR statistic at $t$ is
\begin{equation}
    \mathcal{R}_{Gaussian}(t;[0,T]) = \frac{t(T-t)}{T}\|\hat{\bbrmu}_{(0,t)}-\hat{\bbrmu}_{[t,T]}\|_2^2.
\end{equation}
where $\hat{\bbrmu}_{(0,t)} = \frac{1}{t}\sum_{s=1}^{t-1}Y_s$ and $\hat{\bbrmu}_{[t,T]} = \frac{1}{t}\sum_{s=t}^{T}Y_s$ are maximized likelihood estimators.

Borda count is a popular method for ranking because of its simple and efficient implementation and good performance \citep{shah2017simplerobustrankpairwisecomps, heckel2019activerankingpairwisecomps}. For a given interval $\mathcal{I}$, the Borda count vector $\bbrbeta(\mathcal{I})$ is defined as
\begin{equation}
    \beta(\mathcal{I})_i = N_w(i;\mclI) - N_l(i;\mclI),\forall i\in [n],
\end{equation}
where $N_w(i;\mclI)$ and $N_l(i;\mclI)$ are the number of wining and loss of item $i$ in comparisons over the interval $\mclI$. To apply Borda count to change point detection, we can define $\mathcal{R}_{Borda}(t;(0,T])$ as
\begin{equation}
    \mathcal{R}_{Borda}(t;(0,T]) = \frac{t(T-t)}{T}\|\bbrbeta((0,t))-\bbrbeta([t,T])\|_2^2,
\end{equation}
and $\mathcal{R}_{rank}(t;(0,T])$ as
\begin{equation}
    \mathcal{R}_{rank}(t;(0,T]) = {\rm dis}(\pi(\bbrbeta((0,t))), \pi(\bbrbeta([t,T]))),
\end{equation}
where $\pi(\mathbf{v})$ is the ranking vector of $\mathbf{v}$, and ${\rm dis}(\mathbf{r}_1,\mathbf{r}_2)$ is the distance between two ranking vectors $\mathbf{r}_1, \mathbf{r}_2$. The ranking vector $\pi(\mathbf{v})$ is a permutation of $[n]$ such that $\pi(\mathbf{v})_i$ is the ranking of $v_i$ among all entries of $\mathbf{v}$.

\paragraph{Settings.} We can use $\bbrtheta^*(0)$ and $\bbrtheta^*(\eta)$ to represent the value of true parameters before and after the single change point. For $i> 1$, we set $\theta^*(0)_i = \theta^*(0)_1 +(i -1)\delta$ with some constant $\delta$. We consider three settings of strong-signal changes:

Change I (reverse): $\theta^*(\eta)_i = \theta^*(0)_{n - i}$.

Change II (block exchange): $\theta^*(\eta)_i = \theta^*(0)_{[\frac{n}{2}] + i}$ for $i\leq [\frac{n}{2}]$; $\bbrtheta^*(\eta)_i = \theta^*(0)_{i - [\frac{n}{2}]}$ for $i> [\frac{n}{2}]$.

Change III (reverse $+$ block exchange): $\theta^*(\eta)_i = \theta_{[\frac{n}{2}] + i}$ for $i\leq [\frac{n}{2}]$; $\theta^*(\eta)_i = \theta_{i - [\frac{n}{2}]}$ for $i> [\frac{n}{2}]$ where $\theta_i = \theta^*(0)_{n - i}$.

\paragraph{Results.} We compare the performance of the screening method based on $\mclR_{BT}, \mclR_{Borda}$, and $\mclR_{rank}$. The results are summarized in \Cref{tab0:compare_single_cp}. As we can see from the table, although the two heuristic methods based on $\mclR_{Borda}$ and $\mclR_{rank}$ are fast to apply, their localization errors are much worse than the model-based method $\mclR_{BT}$.
\begin{table}[!ht]
    \centering
    \begin{tabular}{c|cc|cc|cc}
    \hline
    \multicolumn{7}{c}{$n = 10, \Delta = 500, T = 2\Delta$} \\
    \hline
    Change & \multicolumn{2}{c|}{ I} & \multicolumn{2}{c|}{ II}
    & \multicolumn{2}{c}{ III} \\
    \hline
        $\mclR_{BT}$ & 4.5 (4.2)  &  2.97s (0.07)  & 3.8 (4.5)  &  2.91s (0.06)  & 12.3 (10.6) & 2.97s (0.08) \\
    $\mclR_{Borda}$ & 4.6 (3.4) &  0.01s (0.00)  & 9.2 (16.5) & 0.01s (0.00)  & 16.2 (12.2) & 0.01s (0.00) \\
   $\mclR_{rank}$ & 175.9 (99.7) & 0.09s (0.00)  & 186.3 (134.0)  & 0.09s (0.00)  & 328.2 (135.7) & 0.09s (0.00) \\
    \hline
    \multicolumn{7}{c}{$n = 20, \Delta = 500, T = 2\Delta$} \\
    \hline
    Change & \multicolumn{2}{c|}{ I} & \multicolumn{2}{c|}{ II}
    & \multicolumn{2}{c}{ III} \\
    \hline
         $\mclR_{BT}$ & 6.5 (9.7) & 4.47s (0.10)  & 5.8 (4.4) & 4.38s (0.05)  & 23.8 (26.7) & 4.44s (0.05) \\
     $\mclR_{Borda}$ & 4.9 (6.0) & 0.01s (0.00)  &  5.9 (5.6) & 0.01s (0.00)  & 19.8 (23.9) & 0.01s (0.00) \\
     $\mclR_{rank}$ & 66.5 (41.3)  & 0.09s (0.00)  &  184.4 (153.3) & 0.10s (0.01) & 317.7 (185.6) & 0.09s (0.02) \\
    \hline
    \multicolumn{7}{c}{$n = 20, \Delta = 2000,T = 2\Delta$} \\
    \hline
    Change & \multicolumn{2}{c|}{ I} & \multicolumn{2}{c|}{ II}
    & \multicolumn{2}{c}{ III} \\
    \hline
         $\mclR_{BT}$ & 2.8 (2.7)  & 23.4s (0.32)  & 14.1 (14.8) & 24.11s (0.74)  & 17.8 (16.0) & 23.46s (0.15) \\
     $\mclR_{Borda}$ & 3.2 (2.0) & 0.04s (0.00) &  15.1 (14.0) & 0.04s (0.00)  & 19.0 (16.9) & 0.04s (0.00) \\
     $\mclR_{rank}$ & 585.2 (338.9) & 0.35s (0.00) &  463.7 (579.8) & 0.39s (0.03)  & 1911.8 (29.6) & 0.36s (0.02) \\
    \hline
    \multicolumn{7}{c}{$n = 40, \Delta = 2000,T = 2\Delta$} \\
    \hline
    Change  & \multicolumn{2}{c|}{ I} & \multicolumn{2}{c|}{ II}
    & \multicolumn{2}{c}{ III} \\
    \hline
         $\mclR_{BT}$ & 7.8 (6.9)  & 29.29s (0.44)  & 10.7 (12.1)  & 28.92s (0.40) & 30.0 (37.5) & 30.65s (0.73) \\
     $\mclR_{Borda}$ & 7.7 (7.1) & 0.04s (0.00)  & 6.4 (6.2) & 0.04s (0.00) & 59.7 (62.4) & 0.04s (0.00) \\
     $\mclR_{rank}$ & 272.7 & 0.36s (0.01)  & 443.9 (624.7)  & 0.37s (0.02) & 1711.1 (369.5) & 0.37s (0.02) \\
    \hline
    \multicolumn{7}{c}{$n = 100, \Delta = 500,T = 2\Delta$} \\
    \hline
    Change & \multicolumn{2}{c|}{ I} & \multicolumn{2}{c|}{ II}
    & \multicolumn{2}{c}{ III} \\
    \hline
         $\mclR_{BT}$ & 6.1 (7.9) & 9.10s (0.22)  &  19.0 (18.5) & 8.94s (0.25)  & 111.8 (120.7) & 9.07s (0.19) \\
     $\mclR_{Borda}$ & 12.7 (11.7) & 0.01s (0.00)  & 20.7 (22.8) & 0.01s (0.00)  & 236.1 (157.7) & 0.01s (0.00) \\
     $\mclR_{rank}$ & 21.2 (16.3) & 0.10s (0.01)  & 126.4 (146.5) & 0.10s (0.00) & 374.8 (119.7) & 0.10s (0.01) \\
    \hline 
    \multicolumn{7}{c}{$n = 200, \Delta = 500,T = 2\Delta$} \\
    \hline
    Change & \multicolumn{2}{c|}{ I} & \multicolumn{2}{c|}{ II}
    & \multicolumn{2}{c}{ III} \\
    \hline
         $\mclR_{BT}$ & 11.4 (5.6) & 11.25s (0.36)  & 28.9 (37.1) & 11.28s (0.32) & 74.1 (63.7) & 11.79s (0.50) \\
     $\mclR_{Borda}$ & 8.1 (9.7) & 0.01s (0.00) & 21.6 (23.4) & 0.01s (0.00) & 183.7 (171.1) & 0.01s (0.00) \\
     $\mclR_{rank}$ & 16.7 (15.7) & 0.11s (0.00)  & 436.0 (38.7) & 0.11s (0.01) & 448.5 (36.2) & 0.11s (0.01) \\
    \hline    
    \end{tabular}
    \caption{Comparison of GLR and Borda in the single-change-point scenario. Each cell is the average of 10 trials, with the standard error shown in the bracket.}
    \label{tab0:compare_single_cp}
\end{table}


\paragraph{Some thoughts on why $\mclR_{Borda}$ works well} $\mclR_{Borda}$ defined as
\begin{equation}
    \mathcal{R}_{Borda}(t;(0,T]) = \frac{t(T-t)}{T}\|\bbrbeta((0,t))-\bbrbeta([t,T])\|_2^2
\end{equation}
treats the Borda count vectors $\bbrbeta$ as generated from Gaussian mean models and perform well in experiments. 
\begin{equation}
    \beta(\mathcal{I})_i = N_w(i;\mclI) - N_l(i;\mclI),\forall i\in [n],
\end{equation}
where $N_w(i;\mclI)$ and $N_l(i;\mclI)$ are the number of wining and loss of item $i$ in comparisons over the interval $\mclI$. 
A reason could be that, if there is no change point, then the Borda count vector have subgaussian entries with mean
\begin{equation}
    \mathbb{E}[\beta_i(\bbrtheta)] = \frac{2}{n(n-1)}\sum_{j\neq i}\frac{1 - e^{\theta_j - \theta_i}}{1 + e^{\theta_j - \theta_i}}.
\end{equation}
When $\bbrtheta$ changes, it is very likely that $\mathbb{E}[\bbrbeta]$ also changes.



\bnprop
\label{prop:bt_single_cp}
\enprop

\bnprop
\label{prop:multi-Gaussian}
\enprop










\subsection{Multiple change points: DP is the best}
When there are multiple change points, 

We consider $T = 4\Delta$ and three evenly spaced change points $\eta_i = i \Delta$ for $i= 1,2,3$. The changes at $\eta_1,\eta_2,\eta_3$ in contrast to $\bbrtheta^*(0)$ corresponds to the three strong-signal changes described in \Cref{sec0:experiment_single_cp}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{c|cc|cc|cc}
    \hline
    & \multicolumn{2}{c|}{$n = 10, \Delta = 500$} & \multicolumn{2}{c|}{$n = 20, \Delta = 1000$}
    & \multicolumn{2}{c}{$n = 20, \Delta = 2000$} \\
    \hline
    DP &  13.0 (13.1) & 24.53s (1.33)  &  16.0 (20.6) & 120.68s (7.13)  & 18.0 (32.2) & 163.20s (8.59) \\
    WBS-mean & 33.1 (78.0) & 8.08s (0.48)  & 27.8 (41.7) & 25.30s (1.67) & 24.1 (26.6) & 38.22s (4.21) \\
    WBS-GLR &  & s  &  & s  &  & s \\
    WBS-Borda & 48.6 (85.6) & 8.86s (0.50)  & 57.4 (95.0)  &  48.22s (2.26)  & 41.4 (152.6) & 34.28s (3.67) \\
    \hline
    \end{tabular}
    \caption{Comparison of four methods in the multiple-change-points scenario.}
    \label{tab1:compare_single_cp}
\end{table}










\paragraph{Previous settings:}

\begin{table}[!ht]
 \centering
 \begin{tabular}{m{2cm}|m{2cm}m{2cm}|C{1.5cm}C{1.5cm}C{1.5cm}}
 \hline
 \multicolumn{6}{c}{{\bf Setting (i)} \ \ $n = 10, K = 3, \Delta = 500$, Change (I, II, III)} \\
 \hline
 & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\
 DPLR & 32.1 (55.2) & 33.2s (1.0) & 1 & 99 & 0 \\
 WBS-GLR & 52.0 (117.8) & 37.5s (4.7) & 6 & 93 & 1 \\
 \hline
 \multicolumn{6}{c}{ {\bf Setting (ii)} \ \ $n = 20, K = 3, \Delta = 800$, Change (I, II, III)} \\
 \hline
 & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\

 DPLR & 25.3 (27.8) & 109.0s (2.1) & 0 & 99 & 1 \\
 WBS-GLR & 189.8 (221.3) & 147.5s (16.1) & 0 & 61 & 39 \\
 \hline
 \multicolumn{6}{c}{{\bf Setting (iii)}\ \ $n = 100, K = 2, \Delta = 1000$, Change (I, II)} \\
 \hline
 & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\

 DPLR & 41.0 (108.0) & 183.0s (5.5) & 1 & 99 & 0 \\
 WBS-GLR & 156.6 (230.6) & 87.5s (8.3) & 0 & 76 & 24 \\
 \hline
 \multicolumn{6}{c}{{\bf Setting (iv)} \ \ $n = 100, K = 3, \Delta = 2000$, Change (I, II, III)} \\
 \hline
 & $H(\hat{\eta},\eta)$ & Time & $\hat{K}<K$ &$\hat{K}=K$ &$\hat{K}>K$
 \\

 DPLR & 46.8 (88.0) & 403.1s (6.6) & 0 & 100 & 0 \\
 WBS-GLR & 605.2 (494.2) & 282.6s (27.6) & 1 & 35 & 64 \\
 \hline
 \end{tabular}
 \caption{Comparison of DPLR and WBS-GLR under four different simulation settings. 100 trials are conducted in each setting. For the localization error and running time, the average over 100 trials is shown with standard error in the bracket. The three columns on the right record the number of trials in which $\hat{K}<K$, $\hat{K}=K$, and $\hat{K}>K$ respectively.}
 \label{tab:compare_methods_v0}
\end{table}

==> 08_app_backup.tex <==
\section{Applications: backup}
\label{sec:app_backup}

% {\color{red}This is a backup for our own reference. We include six additional teams that were founded between 1976 and 1990, including Heat who eventually became the champion in around S2011.}


We consider the game records of the National Basketball Association (NBA) from season 1976-1977 to season 2015-2016 \footnote{\url{https://gist.github.com/masterofpun/2508ab845d53add72d2baf6a0163d968}}. Usually a regular NBA season begins in October and ends in April of the next year, so a season is referred to by the two years it spans over. The original data contains all game records of NBA from season 1946-1947 to season 2015-2016. We focus on a subset of 18 teams that were founded before 1977 and seasons from season 1976-1977 to season 2015-2016. Our code is available online with the data\footnote{\url{https://anonymous.4open.science/r/CPD_BT-4664}}. 

We start with an exploratory data analysis by calculating the path of the logarithm of generalized likelihood ratio statistics, as is shown in \Cref{fig:nba_glr}. It should be noted that although it looks like the GLR path suggests the existence of two change points, we cannot rely on it, because when multiple change points exist, there will be some cancel-out effect and GLR path may not give consistent estimates of change points \citep{Venkatraman1992}. Here the useful information from the GLR path is that splitting the data by odd and even indices is reasonable. Then we apply our method DPLR to the dataset. We use the samples with odd time indices as training data and even time indices as test data, and use cross-validation to choose the tuning parameter $\gamma$. 


\begin{figure}[H]
    \centering
    \includegraphics[width = 0.31 \textwidth]{figure/nba_glr_all.png}
    \includegraphics[width = 0.31 \textwidth]{figure/nba_glr_odd.png}
    \includegraphics[width = 0.31 \textwidth]{figure/nba_glr_even.png}
    \caption{Path of (logarithmic) generalized loglikelihood ratio on NBA data. Left: GLR path on all samples; mid: GLR path on samples with odd indices; right: GLR path on samples with even indices.}
    \label{fig:nba_glr}
\end{figure}


To interpret the estimated change points, we fit the Bradley-Terry model on the subsets splitted by change point estimates separately. The result is summarized in \Cref{tab:nba_1}. Several teams show significant jumps in the preference scores around the change points. \textcolor{blue}{Can we say something like: 
1990 is the year that Michael Jordan start to dominate the league. 1998 is the year Michael Jordan retired. 1998-2012 is the time   when Spurs and Lakers were dominating the leagues. The two teams together won 9 champions during these seasons.   From  2013  with the arise of super stars   Stephen Curry and Klay Thompson, Golden State Warriors started to dominate the league.}

\begin{table}[!ht]
\centering
\scalebox{0.9}{
\begin{tabular}{lrlrlrlr}
\hline
\multicolumn{2}{c}{\textbf{1976-1990}} & \multicolumn{2}{c}{\textbf{1990-1998}} & \multicolumn{2}{c}{\textbf{1998-2013}} & \multicolumn{2}{c}{\textbf{2013-2015}} \\
\hline
Lakers                & 0.7537         & Bulls                 & 0.8569         & Spurs                 & 0.7995         & Warriors              & 1.3073         \\
Celtics               & 0.5453         & Jazz                  & 0.7317         & Lakers                & 0.5013         & Spurs                 & 1.1567         \\
76ers                 & 0.5257         & Suns                  & 0.5068         & Suns                  & 0.2846         & Trail Blazers         & 0.6193         \\
Bucks                 & 0.2994         & Rockets               & 0.4731         & Jazz                  & 0.1959         & Rockets               & 0.5977         \\
Trail Blazers         & 0.2256         & Knicks                & 0.4002         & Rockets               & 0.1709         & Bulls                 & 0.5283         \\
Suns                  & 0.1360          & Spurs                 & 0.3788         & Pacers                & 0.0630          & Cavaliers             & 0.4268         \\
Nuggets               & 0.0581         & Trail Blazers         & 0.3432         & Trail Blazers         & 0.0564         & Pacers                & 0.1050          \\
Pistons               & 0.0032         & Cavaliers             & 0.3259         & Nuggets               & 0.0362         & Jazz                  & 0.0356         \\
Spurs                 & 0.0001         & Lakers                & 0.1248         & Kings                 & 0.0262         & Celtics               & -0.1222        \\
Rockets               & -0.0343        & Pacers                & 0.0177         & Pistons               & -0.0073        & Nets                  & -0.1237        \\
Jazz                  & -0.1285        & Pistons               & -0.2519        & Celtics               & -0.0406        & Pistons               & -0.1531        \\
Bulls                 & -0.1579        & Warriors              & -0.2906        & 76ers                 & -0.0791        & Suns                  & -0.2754        \\
Knicks                & -0.2012        & Nets                  & -0.3521        & Bucks                 & -0.2730         & Kings                 & -0.3145        \\
Warriors              & -0.3253        & Celtics               & -0.3725        & Bulls                 & -0.2883        & Bucks                 & -0.3544        \\
Pacers                & -0.3882        & Bucks                 & -0.5743        & Cavaliers             & -0.2932        & Nuggets               & -0.4081        \\
Kings                 & -0.3910         & Kings                 & -0.6499        & Knicks                & -0.3645        & Knicks                & -0.5190         \\
Cavaliers             & -0.4391        & Nuggets               & -0.6891        & Nets                  & -0.3830         & Lakers                & -0.9325        \\
Nets                  & -0.4818        & 76ers                 & -0.9788        & Warriors              & -0.4051        & 76ers                 & -1.5737      \\
\hline
\end{tabular}
}
\caption{Fitted $\hat{\bbrtheta}$ on 18 selected teams in 1976-2015 of the National Basketball Association games. The teams are ranked by the MLE $\hat{\bbrtheta}$ on subsets split by three estimated change points given by the DPLR method.}
\label{tab:nba_1}
\end{table}


To close this section, we make a quick discussion on why it's not a good idea to fit \btl{} model on each season and then look for change points. 



\begin{figure}[H]
    \centering
    \includegraphics[width = 0.8 \textwidth]{figure/theta_path.png}
    \caption{Path of $\hat{\bbrtheta}(\mclI_s)$ for $\mclI_s$ being each season of the NBA data.}
    \label{fig:nba_theta_path}
\end{figure}

{\color{red} Another version is included in \Cref{sec:app_backup} for our own use. Some fans of NBA may feel like S1998-S2013 is too big to be a stationary interval. So the other version might look more reasonable. The table there is longer, but we can move some some figures into the appendix to make some space.}

==> 90_checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \Cref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the end of \Cref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \Cref{sec:bt}}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See \Cref{sec:appendix}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See \Cref{sec:experiment,sec:application} for details including a link to our anonymized reproducible code repository
    \ie \url{https://anonymous.4open.science/r/CPD_BT-4664}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \Cref{sec:experiment}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report standard errors of 100 trials, see \Cref{sec:experiment}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the second paragraph of \Cref{sec:experiment}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited all relevant works of the algorithms we used at places they first occur in our paper. We also cite the collector of the data we used in \Cref{sec:application}.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> 99_application_old.tex <==
\clearpage
\section{Application: old results}

\subsection{NFL}

We consider the game records of National Football League (NFL) from season 2009 to season 2015 \footnote{\url{https://www.kaggle.com/datasets/maxhorowitz/nflplaybyplay2009to2016}}. There are 32 teams in NFL playing 16 rounds of games in each season, and in each round there are 16 games so that each team plays only one game. In season 2012, 2013, and 2014, there was one additional game. Thus the total number of games in the dataset is 1,795. Our code is available online with the data\footnote{\url{https://anonymous.4open.science/r/CPD_BT-4664}}.

We start with an exploratory data analysis by calculating the path of the logarithm of generalized likelihood ratio statistics. The result is shown in \Cref{fig:nfl_glr}. The GLR path indicates that there might be a change point aground index 900,
{\color{blue}  The estimated change point of DPLR is 622. They differ by around 300. However, in figure 1, it seems that the second and the third objective function is maximized at around 450. } or equivalently, the mid of season 2012. {\color{red} To Ale: do we need to put some discussions on why GLR ``partly" works (i.e., works for single change point but if multiple change points exist then there will be some issue) in the appendix and make a cross-ref here?}

Then, we apply our method DPLR to the dataset. As we have done in simulations, we use the samples with odd time indices as training data and even time indices as test data, and use cross-validation  to choose the tuning parameter $\gamma$.  DPLR gives a single change point $\tilde{\eta} = 311$ in the subsets, or $\hat{\eta} = 622$ in the original data, which corresponds to mid season 2011. This does not differ a lot from the heuristic estimation based on the GLR path.

\begin{figure}[H]
    \centering
    \includegraphics[width = 0.31 \textwidth]{figure/nfl_glr_all.png}
    \includegraphics[width = 0.31 \textwidth]{figure/nfl_glr_odd.png}
    \includegraphics[width = 0.31 \textwidth]{figure/nfl_glr_even.png}
    \caption{Path of (logarithmic) generalized loglikelihood ratio on NFL data. Left: GLR path on all samples; mid: GLR path on samples with odd indices; right: GLR path on samples with even indices.}
    \label{fig:nfl_glr}
\end{figure}


\begin{table}[!h]
\centering
\begin{tabular}{m{4cm}R{2.5cm}R{2.5cm}R{2.5cm}}
\hline
{Team} & $\hat{\bbrtheta}((0,T])$ &  $\hat{\bbrtheta}(1)$ & $\hat{\bbrtheta}(\hat{\eta})$ \\
\hline
New England Patriots            & 1.1304            & 1.3331          & 1.1413           \\
Green Bay Packers            & 0.8067            & 0.9422          & 0.7737          \\
Pittsburgh Steelers           & 0.5288              & 0.7817          & 0.4390          \\
\rowcolor{blue!25}
Denver Broncos           & 0.5185            & -0.5324         & 1.1434           \\
\rowcolor{yellow!25}
New Orleans Saints            & 0.4406            & 1.0754          & 0.1447          \\
Cincinnati Bengals           & 0.4227            & 0.0911          & 0.6442          \\
Baltimore Ravens           & 0.4190            & 0.8366          & 0.2504          \\
\rowcolor{blue!25}
Seattle Seahawks           & 0.3262            & -0.8270         & 1.0230          \\
Indianapolis Colts           & 0.2891            & 0.4358          & 0.1752          \\
\rowcolor{yellow!25}
San Francisco 49ers            & 0.2778            & -0.2078         & 0.5847           \\

Atlanta Falcons           & 0.2567             & 0.7778          & -0.0263         \\
\rowcolor{blue!25}
Arizona Cardinals           & 0.2283            & -0.6616         & 0.7247          \\
Philadelphia Eagles           & 0.0857            & 0.4383           & -0.0612         \\
\rowcolor{yellow!25}
Los Angeles Chargers           & 0.0796            & 0.5855          & -0.2439         \\
\rowcolor{blue!25}
Carolina Panthers           & 0.0717             & -0.7067         & 0.4474          \\
Chicago Bears           & 0.0382            & 0.3112         & -0.0789         \\
Minnesota Vikings           & 0.0149            & -0.0191         & 0.0446          \\
\rowcolor{yellow!25}
New York Jets           & 0.0141            & 0.6594          & -0.2915         \\
Dallas Cowboys           & -0.0041           & 0.0562          & -0.0022           \\
New York Giants           & -0.0617           & 0.2174          & -0.2547         \\
Houston Texans           & -0.0866           & -0.0413         & -0.1375         \\
Kansas City Chiefs            & -0.1001           & -0.2801         & -0.0148         \\
Miami Dolphins           & -0.2142           & -0.3325         & -0.1198         \\
Detroit Lions           & -0.2336           & -0.6672         & -0.0119         \\
Buffalo Bills           & -0.3787           & -0.3053         & -0.3886         \\
Washington Commanders           & -0.5873           & -0.8020         & -0.5502          \\
Las Vegas Raiders           & -0.6056            & -0.3261         & -0.8396         \\
\rowcolor{blue!25}
Los Angeles Rams           & -0.6248           & -1.5435         & -0.1850         \\
Tennessee Titans           & -0.6366           & -0.2298         & -0.9446         \\
Tampa Bay Buccaneers            & -0.6981            & -0.1830         & -1.0575         \\
Cleveland Browns           & -0.7964           & -0.5726         & -0.9356         \\
\rowcolor{yellow!25}
Jacksonville Jaguars           & -0.9215          & -0.3039         & -1.3925     \\
\hline
\hspace{0.2cm}
\end{tabular}

\caption{Fitted $\hat{\bbrtheta}$ on NFL data 2009-2015, rounded to the fourth decimal. The estimated change point is in season 2011. $\hat{\bbrtheta}((0,T])$ is the MLE fitted on all samples with $T = 1795$. $\hat{\eta} = 622$ and $\hat{\bbrtheta}(1)$, $\hat{\bbrtheta}(\hat{\eta})$ are the MLE on two subsets splitted at the estimated change point $\hat{\eta}$. Teams with top-5 score increase are marked in blue, and teams with top-5 score decrease are marked in yellow.}
\label{tab:nfl}
\end{table}

To interpret the estimated change point $\hat{\eta} = 622$, we fit a joint Bradley-Terry model on the original data and get $\hat{\bbrtheta}((0,T])$, and two Bradley-Terry models on the two subsets splitted at $\hat{\eta}$ separately. The result is summarized in \Cref{tab:nfl}. The jumps in the preference scores of many teams support our conclusion that there is a change point around $\hat{\eta} = 622$. Some events happened in season 2011 and 2012 may give more evidence for such change. {\color{red} I am trying to organize some info from wiki on relevant events}.







% \begin{table}[!h]
% \centering
% \begin{tabular}{m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
% \hline
% {Team} & $\hat{\bbrtheta}((0,T])$ &  $\hat{\bbrtheta}(0)$ & $\hat{\bbrtheta}(\hat{\eta})$ \\
% \hline
% NE            & 1.130439            & 1.333079          & 1.14131           \\
% GB            & 0.806659            & 0.942213          & 0.773701          \\
% PIT           & 0.5288              & 0.781693          & 0.438962          \\
% \rowcolor{blue!25}
% DEN           & 0.518507            & -0.532437         & 1.14342           \\
% \rowcolor{yellow!25}
% NO            & 0.440646            & 1.075395          & 0.144659          \\
% CIN           & 0.422672            & 0.091102          & 0.644207          \\
% BAL           & 0.418957            & 0.836628          & 0.250366          \\
% \rowcolor{blue!25}
% SEA           & 0.326165            & -0.826989         & 1.022987          \\
% IND           & 0.289068            & 0.435778          & 0.175208          \\
% \rowcolor{yellow!25}
% SF            & 0.277844            & -0.207775         & 0.58473           \\

% ATL           & 0.25668             & 0.777759          & -0.026284         \\
% \rowcolor{blue!25}
% ARI           & 0.228255            & -0.661585         & 0.724699          \\
% PHI           & 0.085688            & 0.43826           & -0.061205         \\
% \rowcolor{yellow!25}
% SD            & 0.079635            & 0.585535          & -0.243945         \\
% \rowcolor{blue!25}
% CAR           & 0.07186             & -0.706668         & 0.447435          \\
% CHI           & 0.038189            & 0.311258          & -0.078942         \\
% MIN           & 0.014893            & -0.019065         & 0.044636          \\
% \rowcolor{yellow!25}
% NYJ           & 0.014142            & 0.659404          & -0.291504         \\
% DAL           & -0.004116           & 0.056179          & -0.0022           \\
% NYG           & -0.061666           & 0.217414          & -0.254746         \\
% HOU           & -0.086569           & -0.041284         & -0.137536         \\
% KC            & -0.100111           & -0.280085         & -0.014791         \\
% MIA           & -0.214192           & -0.33247          & -0.119759         \\
% DET           & -0.233553           & -0.667196         & -0.011872         \\
% BUF           & -0.378689           & -0.305252         & -0.388566         \\
% WAS           & -0.587287           & -0.802015         & -0.55021          \\
% OAK           & -0.60564            & -0.326061         & -0.839583         \\
% \rowcolor{blue!25}
% STL           & -0.624759           & -1.543485         & -0.185025         \\
% TEN           & -0.636585           & -0.229768         & -0.944612         \\
% TB            & -0.69806            & -0.183042         & -1.057455         \\
% CLE           & -0.796368           & -0.572607         & -0.935577         \\
% \rowcolor{yellow!25}
% JAC           & -0.921506           & -0.303914         & -1.392507     \\
% \hline
% \hspace{0.2cm}
% \end{tabular}

% \caption{Fitted $\hat{\bbrtheta}$ on NFL data 2009-2015. The estimated change point is in season 2011. $\hat{\bbrtheta}((0,T])$ is the MLE fitted on all samples with $T = 1795$. $\hat{\eta} = 622$ and $\hat{\bbrtheta}(0)$, $\hat{\bbrtheta}(\hat{\eta})$ are the MLE on two subsets splitted at the estimated change point $\hat{\eta}$. Teams with top-5 score increase are marked in blue, and teams with top-5 score decrease are marked in yellow.}
% \label{tab:nfl}
% \end{table}



\subsection{International football games}
We use a dataset of game records of international men football games from 1872 to 2022\footnote{\url{https://www.kaggle.com/datasets/martj42/international-football-results-from-1872-to-2017}}. The original dataset contains 43,170 games involving 304 national football teams. For more accurate inference, we focus on games after 1950 and 30 teams with top rankings according to FIFA. In addition, we remove teams that had their first game record later than 1955 and end up with 20 teams and 2,773 games.







\begin{table}[!h]
\centering
\begin{tabular}{rrrrrr}
\hline
Team & $\hat{\bbrtheta}((0,T])$ & Team & $\hat{\bbrtheta}(0)$ & Team & $\hat{\bbrtheta}(\hat{\eta})$ \\
\hline
Brazil        & 0.94147             & Brazil           & 1.306498          & Brazil           & 0.879032          \\
Argentina     & 0.650869            & \cellcolor{yellow!25}Italy            & 1.288201          & \cellcolor{blue!25}France           & 0.66482           \\
\cellcolor{yellow!25}Italy         & 0.556338            & \cellcolor{yellow!25}England          & 1.033289          & Spain            & 0.655063          \\
Spain         & 0.541973            & Argentina        & 0.914063          & Argentina        & 0.642057          \\
Germany       & 0.477933            & Germany          & 0.690592          & Germany          & 0.449398          \\
\cellcolor{yellow!25}England       & 0.397763            & Uruguay          & 0.603852          & \cellcolor{yellow!25}Italy            & 0.411665          \\
\cellcolor{blue!25}France        & 0.394005            & Sweden           & 0.366106          & \cellcolor{blue!25}Netherlands      & 0.369605          \\
\cellcolor{blue!25}Netherlands   & 0.120653            & Spain            & 0.310855          & \cellcolor{yellow!25}England          & 0.162192          \\
Uruguay       & 0.083346            & Chile            & -0.01607          & Portugal         & 0.095077          \\
Belgium       & 0.018637            & Belgium          & -0.040897         & Uruguay          & -0.022534         \\
Sweden        & -0.033973           & Peru             & -0.147429         & Belgium          & -0.095331         \\
Portugal      & -0.051007           & Mexico           & -0.225761         & Chile            & -0.18682          \\
Chile         & -0.196591           & \cellcolor{blue!25}France           & -0.327218         & Sweden           & -0.197241         \\
Mexico        & -0.334121           & Portugal         & -0.352993         & Denmark          & -0.316626         \\
Switzerland   & -0.389168           & Switzerland      & -0.405107         & Mexico           & -0.348069         \\
Denmark       & -0.41697            & Egypt            & -0.530753         & Switzerland      & -0.431454         \\
Peru          & -0.454929           & Wales            & -0.624824         & Peru             & -0.486281         \\
Egypt         & -0.689182           & \cellcolor{blue!25}Netherlands      & -0.695561         & Egypt            & -0.711178         \\
Wales         & -0.767581           & Denmark          & -0.879119         & Wales            & -0.756823         \\
United States & -0.849465           & United States    & -2.267727         & United States    & -0.776549        \\
\hline
\hspace{0.2cm}
\end{tabular}
\caption{Fitted $\hat{\bbrtheta}$ on 20 teams in 1950-2022 of International bootball data. The estimated change point $\hat{\eta}$ is in year 1970. $\hat{\bbrtheta}((0,T])$ is the MLE fitted on all samples. $\hat{\bbrtheta}(0)$ and $\hat{\bbrtheta}(\hat{\eta})$ are the MLE on two subsets split by the estimated change point $\hat{\eta}$. Two teams with biggest ranking and score increase are marked in blue, and two teams with ranking and score decrease are marked in yellow.}
\end{table}













% \begin{table}[H]
% \centering
% \begin{tabular}{m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
% \hline
% {Team} & $\hat{\bbrtheta}((0,T])$ &  $\hat{\bbrtheta}(0)$ & $\hat{\bbrtheta}(\hat{\eta})$ \\
% \hline
% Brazil        & 0.94147             & 1.306498          & 0.879032          \\
% Argentina     & 0.650869            & 0.914063          & 0.642057          \\
% Italy         & 0.556338            & 1.288201          & 0.411665          \\
% Spain         & 0.541973            & 0.310855          & 0.655063          \\
% Germany       & 0.477933            & 0.690592          & 0.449398          \\
% \rowcolor{yellow!25}
% England       & 0.397763            & 1.033289          & 0.162192          \\
% \rowcolor{blue!25}
% France        & 0.394005            & -0.327218         & 0.66482           \\
% \rowcolor{blue!25}
% Netherlands   & 0.120653            & -0.695561         & 0.369605          \\
% Uruguay       & 0.083346            & 0.603852          & -0.022534         \\
% Belgium       & 0.018637            & -0.040897         & -0.095331         \\
% Sweden        & -0.033973           & 0.366106          & -0.197241         \\
% Portugal      & -0.051007           & -0.352993         & 0.095077          \\
% Chile         & -0.196591           & -0.01607          & -0.18682          \\
% Mexico        & -0.334121           & -0.225761         & -0.348069         \\
% Switzerland   & -0.389168           & -0.405107         & -0.431454         \\
% Denmark       & -0.41697            & -0.879119         & -0.316626         \\
% Peru          & -0.454929           & -0.147429         & -0.486281         \\
% Egypt         & -0.689182           & -0.530753         & -0.711178         \\
% Wales         & -0.767581           & -0.624824         & -0.756823         \\
% \rowcolor{blue!25}
% United States & -0.849465           & -2.267727         & -0.776549        \\
% \hline
% \end{tabular}
% \end{table}
